On the Impact of Finite-Length Probabilistic Shaping on Fiber Nonlinear Interference

The interplay of shaped signaling and fiber nonlinearities is reviewed in the asymptotic and finite-length regime. We present explanations and discuss implications of an optimum shaping length of just a few hundred symbols.

==> myFigures.tex <==
%% Graphics
\usepackage{color}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikzscale}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{plotmarks,matrix,chains,scopes,fit,calc,shapes,positioning,decorations,intersections,fit,backgrounds,patterns}
\pgfplotsset{compat=newest} 

%% tikz externalize
% \usepgfplotslibrary{external}
% \tikzexternalize % activate with a name prefix
% \tikzsetexternalprefix{tikz/}
% \tikzsetfigurename{tikz} % set name of figure
% \tikzset{external/up to date check=md5}

%% tikz
\pgfplotsset{plot coordinates/math parser=false}
% \pgfplotsset{every axis/.append style={font=\footnotesize}}
\pgfplotsset{every axis plot/.append style={solid,line width=1.5pt,mark size=1.5pt,mark options={solid,fill=white}}}
% \pgfplotsset{every axis plot/.append style={solid,line width=1pt,mark size=2pt,mark options={solid,fill=white}}}
\pgfplotsset{every axis legend/.append style={legend cell align=left,font=\footnotesize}}



%% colors
\colorlet{42GBd16QAM_color}{blue!80!white}
\colorlet{42GBd64QAM_color}{red!80!black}
\colorlet{42GBd64QAMnoNL_color}{blue!80!white}
\colorlet{64GBd64QAM_color}{gray!50!black}
% \definecolor{64GBd64QAM_color}{rgb}{0.00000,0.58824,0.00000}%
% \definecolor{64GBd16QAM_color}{rgb}{1.00000,0.58824,0.00000}%
% \definecolor{42GBd16QAM_color}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{42GBd16QAM_color}{rgb}{0.50000,0.58824,1.00000}%

%% plot styles
\pgfplotsset{64GBd64QAM/.style={color=64GBd64QAM_color,solid}}
\pgfplotsset{64GBd16QAM/.style={color=64GBd16QAM_color,dotted}}
\pgfplotsset{42GBd64QAM/.style={color=42GBd64QAM_color,solid}}
\pgfplotsset{42GBd64QAMnoNL/.style={color=42GBd64QAMnoNL_color,dashed}}
\pgfplotsset{42GBd16QAM/.style={color=42GBd16QAM_color,dash dot dot}}
% \pgfplotsset{XPM_GaussInput/.style={color=myred,dashed}}
% \pgfplotsset{XPMmodel/.style={color=myred,solid}}
% \pgfplotsset{sims/.style={color=sims,only marks,mark=*,mark options={solid,fill=white,line width=1pt}}}

%% dimensions
\newlength\FigureWidth
\newlength\FigureHeight
\newlength\FullFigureWidth
\setlength\FigureWidth{0.67\textwidth}
\setlength\FullFigureWidth{0.3\textwidth}
\setlength\FigureHeight{0.55\FigureWidth}
\graphicspath{{figures/}}

%% legend
\pgfplotsset{myLegend/.append style={legend style={font=\footnotesize,at={(0.5,0.98)},anchor=north,align=left,legend columns=3}}}


\newcommand{\inputtikz}[1] {% directly input tikz without tikzscale
  % \tikzsetnextfilename{#1}%
  \input{figures/#1.tikz}
}

==> mymacros.tex <==
%% Tobias Fehenberger
%% macros for PhD dissertation

%% Comments
\newcommand{\tf}[1]{\textcolor{red}{\uline{#1}}}
% \renewcommand{\tf}[1]{#1}
\newcommand{\up}[1]{\textcolor{green!50!black}{\uline{#1}}}


%% Fiber Setup
\newcommand{\Nch}{\ensuremath{N_{\textrm{ch}}}\xspace}
\newcommand{\Bch}{\ensuremath{B_{\textrm{ch}}}\xspace}
\newcommand{\Nspans}{\ensuremath{N_{\textrm{spans}}}\xspace}

%% Operators
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}
\newcommand{\Entr}{\ensuremath{\mathbb{H}}}
\newcommand{\entr}{\ensuremath{\mathbb{h}}}
\newcommand{\Real}[1]{\mathbb{R}\{#1\}}
\newcommand{\Imag}[1]{\mathbb{I}\{#1\}}


%% AIR
\newcommand{\Rbmd}{\ensuremath{\text{R}_{\text{BMD}}}\xspace}
\newcommand{\Ibmdhat}{\ensuremath{\hat{I}_{\text{BMD}}}\xspace}
\newcommand{\GMI}{\ensuremath{\text{GMI}}\xspace}
\newcommand{\LLR}{\ensuremath{\text{LLR}}}
\newcommand{\Rsym}{\ensuremath{\text{R}_{\text{SYM}}}\xspace}
\newcommand{\Rsymhat}{\ensuremath{\hat{\text{R}}_{\text{sym}}}\xspace}
\newcommand{\Rloss}{\ensuremath{R_{\text{loss}}}\xspace}
\newcommand{\Rlossn}{\ensuremath{R_{\text{loss},n}}\xspace}
\newcommand{\AIRn}{\ensuremath{\text{AIR}_n}\xspace}

%% RVs
\newcommand{\X}{\ensuremath{X}\xspace}
\newcommand{\Xn}{\ensuremath{X^n}\xspace}
\newcommand{\Y}{\ensuremath{Y}\xspace}
\newcommand{\Yn}{\ensuremath{Y^n}\xspace}
\newcommand{\B}{\ensuremath{\boldsymbol{B}}\xspace}
\newcommand{\setX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\x}{\ensuremath{x}\xspace}
\newcommand{\y}{\ensuremath{y}\xspace}
\newcommand{\bfmu}{\ensuremath{\mu}\xspace}

\newcommand{\momforth}{\standmom{4}\xspace}
\newcommand{\momsixth}{\standmom{6}\xspace}
\newcommand{\kth}{\ensuremath{k^{\text{th}}}\xspace}
\newcommand{\auxch}{\ensuremath{q_{\Y|\X}}\xspace}


%% SNR
\newcommand{\Ptx}{\ensuremath{P_{\text{tx}}}\xspace}
\newcommand{\Ptxopt}{\ensuremath{P_{\text{tx,opt}}}\xspace}
\newcommand{\sigmaASE}{\ensuremath{\sigma^2_{\text{ASE}}}\xspace}
\newcommand{\NoiseEff}{\ensuremath{\sigma^2_{\text{eff}}}\xspace}
\newcommand{\SNREff}{\ensuremath{\text{SNR}_{\text{eff}}}\xspace}
\newcommand{\NoiseNLI}{\ensuremath{\sigma^2_{\text{NLI}}}\xspace}
\newcommand{\NoiseIntra}{\ensuremath{\sigma^2_{\text{NLI,intra}}}\xspace}
\newcommand{\NoiseInter}{\ensuremath{\sigma^2_{\text{NLI,inter}}}\xspace}
\newcommand{\EbN}{\ensuremath{E_\text{b}/N_0}\xspace}
\newcommand{\EsN}{\ensuremath{E_\text{s}/N_0}\xspace}


%% SPM-XPM model
\newcommand{\chiintra}{\ensuremath{\chi_{\text{intra}}}\xspace}
\newcommand{\chiinter}{\ensuremath{\chi_{\text{inter}}}\xspace}
\newcommand{\chiforth}{\ensuremath{\chi_{4}}\xspace}
\newcommand{\chisixth}{\ensuremath{\chi_{6}}\xspace}
\newcommand{\chinomom}{\ensuremath{\chi_{0}}\xspace}
\newcommand{\standmom}[1]{\ensuremath{\hat{\mu}_{#1}}\xspace}

%% short notation
\newcommand{\tento}[1]{$\times$10\textsuperscript{#1}}


%% TODO to sort
\newcommand{\BERin}{\ensuremath{\textrm{BER}_{\textrm{in}}}\xspace}
\newcommand{\BERout}{\ensuremath{\textrm{BER}_{\textrm{out}}}\xspace}
\newcommand{\RSD}{\ensuremath{\textrm{R}_{\textrm{SD}}}\xspace}
\newcommand{\RHD}{\ensuremath{\textrm{R}_{\textrm{HD}}^1}\xspace}
\newcommand{\RHDm}{\ensuremath{\textrm{R}_{\textrm{HD}}^{m}}\xspace}
\newcommand{\RHDone}{\ensuremath{\textrm{R}_{\textrm{HD}}^1}\xspace}
\newcommand{\gammaeff}{\ensuremath{\gamma_\text{eff}}\xspace}

%% units
\newcommand{\unitgamma}{\ensuremath{\frac{1}{\text{W} \cdot \text{km}}}\xspace}

\newcommand{\ASE}{\ensuremath{\sigma^2_{\text{ASE}}}\xspace}
\newcommand{\SNR}{\ensuremath{\text{SNR}_{\text{eff}}}\xspace}
